Identifying Competition and Mutualism Between Online Groups

Platforms often host multiple online groups with overlapping topics and members. How can researchers and designers understand how related groups affect each other? Inspired by population ecology, prior research in social computing and human-computer interaction has studied related groups by correlating group size with degrees of overlap in content and membership, but has produced puzzling results: overlap is associated with competition in some contexts but with mutualism in others. We suggest that this inconsistency results from aggregating intergroup relationships into an overall environmental effect that obscures the diversity of competition and mutualism among related groups. Drawing on the framework of community ecology, we introduce a time-series method for inferring competition and mutualism. We then use this framework to inform a large-scale analysis of clusters of subreddits that all have high user overlap. We find that mutualism is more common than competition.

==> resources/network-figures.tex <==
\begin{figure*}
\begin{minipage}[t][][t]{0.49\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/mental_graphviz.pdf}
  \subcaption{The ecological community of subreddits for supporting mental health and survivors of abuse is dense with largely mutualistic interactions. Some interactions, like that between \texttt{r\Slash mentalhealth} and \texttt{r\Slash survivorsofabuse} are mutualistic in one direction but competitive in the other. \label{fig:mut.network}}
\end{minipage}
\hfill
\begin{minipage}[t][][t]{0.49\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/realestate_graphviz.pdf}
  \subcaption{ The subreddits about real estate and finance are relatively competitive. We detect reciprocal competitive relationships among the real estate subreddits in the triad including   \texttt{r\Slash realestateinvesting}, \texttt{r\Slash realestate} and \texttt{r\Slash commercialrealestate}.  \label{fig:comp.network}}
\end{minipage}
\begin{minipage}[t][][t]{0.49\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/watches_graphviz.pdf}
  \subcaption{Subreddits about watches are dense with both mutualistic and competitive interactions.  There is a reciprocal competitive interaction between \texttt{r\Slash gshock} and \texttt{r\Slash seiko}, a reciprocal mutualistic interaction between \texttt{r\Slash gshock} and \texttt{r\Slash rolex} well as several unreciprocated mutualistic and competitive interactions. \label{fig:mixed.network}}
\end{minipage}
\hfill
\begin{minipage}[t][][t]{0.49\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/cod_graphviz.pdf}
  \subcaption{An ecological community of subreddits about Call of Duty video games characterized by relatively sparse ecological interactions. We detect only two mutualistic interactions from \texttt{r\Slash blackops3} to \texttt{r\Slash infinitewarfare} from codzombies to \texttt{r\Slash infinitewarfare}. \label{fig:void.network}}
\end{minipage}
\caption{Network visualizations of commensal relationships in example ecological communities of subreddits with overlapping users. \textcolor{mycomp}{Yellow} indicates \textcolor{mycomp}{competition} and \textcolor{mymut}{purple} indicates \textcolor{mymut}{mutualism}.  \label{fig:networks}}
\end{figure*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

